No-frills Temporal Video Grounding: Multi-Scale Neighboring Attention and Zoom-in Boundary Detection

Temporal video grounding (TVG) aims to retrieve the time interval of a language query from an untrimmed video. A significant challenge in TVG is the low "Semantic Noise Ratio (SNR)", which results in worse performance with lower SNR. Prior works have addressed this challenge using sophisticated techniques. In this paper, we propose a no-frills TVG model that consists of two core modules, namely multi-scale neighboring attention and zoom-in boundary detection. The multi-scale neighboring attention restricts each video token to only aggregate visual contexts from its neighbor, enabling the extraction of the most distinguishing information with multi-scale feature hierarchies from high-ratio noises. The zoom-in boundary detection then focuses on local-wise discrimination of the selected top candidates for fine-grained grounding adjustment. With an end-to-end training strategy, our model achieves competitive performance on different TVG benchmarks, while also having the advantage of faster inference speed and lighter model parameters, thanks to its lightweight architecture.

==> backup/intro.tex <==
Given a language query, temporal video grounding (TVG) \cite{gao2017CTRL,anne2017TVG1} aims to retrieve the corresponding clip (e.g. represented by frame interval $[t_s, t_e]$) from an untrimmed video (e.g. represented by frame interval $[0,T]$). The semantics of the query normally correspond to only a small portion of the entire long video.
If we define the ``\textbf{semantic noise ratio (SNR)}'' as the ratio of the target clip interval to the untrimmed video interval, i.e. $\mathrm{SNR}=\frac{(t_e-t_s)}{T}$, then the TVG task usually exhibits the property of low SNR.  
As shown in Figure~\ref{fig:intro1}, a large percentage of TVG trials in different benchmarks have low SNR. 
For example, almost all trials in Ego4D-NLQ \cite{grauman2022ego4d} have SNR lower than 0.2. 
We argue that the property of low SNR has been the root of challenges for the TVG task, as it is very challenging for a TVG model to strike a balance between capturing finer-grained spatial-temporal visual information and suppressing noise under the low SNR condition. 
As shown in Figure~\ref{fig:intro1}, when SNR drops from [0.4,0.6] to [0.2,0.4], it leads to a nearly $30\%$ drop in performance on the R1@0.5 metric for state-of-the-art methods \cite{liu2021IANET,zhang20192DTAN}.



\begin{figure}[t]
\begin{center}
	\includegraphics[width=1\linewidth]{imgs/intro1.pdf}
\end{center}
\caption{
\textbf{Bar}: Statistics of SNR distribution in different TVG benchmarks. \textbf{Curve}: Rank1@0.5 accuracy of 2D-TAN and IANet under different SNR on ActivityNet. 
}
\label{fig:intro1}
\end{figure}


In contrast, most trimmed video tasks (e.g., text-video retrieval task~\cite{lin2022swinbert}) typically have high SNR, and thus can effectively employ dense frame sampling to enhance video understanding. However, due to the low SNR, which also implies a semantic asymmetry between the query and the untrimmed video, simply increasing the frame sampling may instead hurt the performance.
As shown in Figure~\ref{fig:ego4d}, for existing TVG methods, with the increase of frame sampling, the performance does not improve but decreases. The best results are actually achieved by sparse sampling (200 frames, around 0.4 FPS). But paradoxically, sparse sampling inevitably leads to the loss of key information.

To alleviate the negative influence of low SNR, increasingly sophisticated techniques have been proposed for the TVG task recently.
For example, CBLN~\cite{liu2021CBLN} proposes a hierarchical multi-branch model to enrich frame representation with multi-contexts. 
CSMGAN~\cite{liu2020CSMGAN} proposes multi-level relation graphs to capture high-order interactions between two modalities.
MSA~\cite{zhang2021MSA} designs a multi-stage aggregated transformer to enhance iterations and alignments among all visual-text elements. IANet~\cite{liu2021IANET} adopts a multi-step calibration module with extra learnable parameters to alleviate the nowhere-to-attend problem of non-matched frame-word pairs. All these solutions involve complex architectures or more parameters that need to be carefully tuned, which hinders their generalization capability. 

In this study, instead of designing complex techniques, we propose a no-frills model for temporal video grounding.
Inspired by human's cognitive habits to retrieve a clip corresponding to a language description, that is, we tend to  first skim the video based on local view to spot the target clip quickly, and then scrutinize the clip boundary carefully, we propose two core modules in our no-frills TVG model, namely multi-scale neighboring attention (MNA) and zoom-in boundary detection (ZBD), which are modest and easy to plug in other existing models. With only light-weight transformer architecture and multi-layer perceptrons (MLPs), our model still achieves competitive performance on a broad range of TVG benchmarks with faster inference speed and lower parameter.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.9\linewidth]{imgs/intro2.pdf}
	\end{center}
	\caption{Rank1@0.3 accuracy results using different number of sampled frames on Ego4D-NLQ. }
	\label{fig:ego4d}
\end{figure}


Specifically, the proposed multi-scale neighboring attention restricts each video token to only aggregate visual contexts from its neighbors, while hierarchically reducing its scope from bottom to top.

It creates a multi-scale pyramid of feature aggregation inside the transformer block, effectively enabling our model to extract most distinguishable information with multi-scale feature hierarchies from high-ratio noises, while refining the extracted semantics throughout the input stream. 
Moreover, we propose a zoom-in boundary detection module, which screens out the top candidates, and then zooms in to focus on local-wise discrimination for fine-grained grounding adjustment. 
 
With all the proposed modules, in contrast to other methods, our model performance can be effectively improved with increasing frame sampling rate as shown in Figure~\ref{fig:ego4d}.



The main contributions of this work include: 
(1) We propose a simple but effective framework for temporal video grounding without bells and whistles;
(2) We propose multi-scale neighboring attention, zoom-in boundary detection to mitigate the interference of noises brought by low SNR of untrimmed videos, resulting in high-quality proposals.
(3) We achieve competitive performance on three widely used benchmarks: ActivityNet, Charades and Ego4D-NLQ.

